SimPO: Simple Preference Optimization with a Reference-Free Reward

Direct Preference Optimization (DPO) is a widely used offline preference optimization algorithm that reparameterizes reward functions in reinforcement learning from human feedback (RLHF) to enhance simplicity and training stability. In this work, we propose SimPO, a simpler yet more effective approach. The effectiveness of SimPO is attributed to a key design: using the average log probability of a sequence as the implicit reward. This reward formulation better aligns with model generation and eliminates the need for a reference model, making it more compute and memory efficient. Additionally, we introduce a target reward margin to the Bradley-Terry objective to encourage a larger margin between the winning and losing responses, further improving the algorithm's performance. We compare SimPO to DPO and its latest variants across various state-of-the-art training setups, including both base and instruction-tuned models such as Mistral, Llama 3, and Gemma 2. We evaluate on extensive chat-based evaluation benchmarks, including AlpacaEval 2, MT-Bench, and Arena-Hard. Our results demonstrate that SimPO consistently and significantly outperforms existing approaches without substantially increasing response length. Specifically, SimPO outperforms DPO by up to 6.4 points on AlpacaEval 2 and by up to 7.5 points on Arena-Hard. Our top-performing model, built on Gemma-2-9B-it, achieves a 72.4% length-controlled win rate on AlpacaEval 2, a 59.1% win rate on Arena-Hard, and ranks 1st on Chatbot Arena among <10B models with real user votes.

==> Rebuttal/alpcaeval.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=\textwidth]{Rebuttal/AlpacaEval.pdf}
\caption{Screenshot of the AlpacaEval 2 leaderboard taken on 08/05/2024. Fine-tuning Gemma-2-9B-IT with \method on on-policy UltraFeedback data results in one of the top-performing models on the leaderboard. \label{fig:ae2_leaderboard}}
\end{figure}


==> Rebuttal/kld.tex <==

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.4\textwidth}
\centering
\raisebox{.0pt}{\includegraphics[width=\textwidth]{Figures/kld_plot.pdf}}
% \vspace{-0.5em}
\caption{KL divergence w/ different $\beta$. \label{fig:rebut_kld}}
\end{subfigure}%
~
\begin{subfigure}[t]{0.4\textwidth}
\centering
\raisebox{.8pt}{\includegraphics[width=\textwidth]{Figures/ae2_different_beta.pdf}}
% \vspace{-0.5em}
\caption{Performance w/ different $\beta$. \label{fig:rebut_ae2_beta}}
\end{subfigure}%
% ~
% \begin{subfigure}[t]{0.328\textwidth}
% \centering
% \raisebox{6.7pt}{\includegraphics[width=\textwidth]{Figures/efficiency_study.pdf}}
% % \vspace{-0.5em}
% \caption{Efficiency of DPO vs. \method. \label{fig:efficiency}}
% \end{subfigure}
\caption{
(a) With different $\beta$ in DPO and \method, KL divergence from the policy model to the reference model on winning responses.
(b) AlpacaEval2 LC win rate of DPO and \method with different $\beta$.
% (c) Runtime and memory usage for DPO and \method.
With proper hyperparameters, \method can result in a similar KL divergence to DPO under its optimal $\beta=0.01$. 
Increasing $\beta$ for DPO (\eg, $\beta=0.1$) reduces KL divergence but also overly constrains training.
}
\vspace{-1em}
\label{fig:kld_rebut} 
\end{figure}

% \begin{figure}[!t]
% \caption{An AlpacaEval 2 generation comparing different model outputs on antenna types.}
% \label{tab:antenna_types}
% { \tt \footnotesize \begin{tabularx}{\linewidth}{r X} \toprule
% \textbf{Input} $\to$ & Q: antennas that transmit an equal amount of energy in the horizontal direction are called  \
% \midrule \textbf{GPT4-turbo} $\to$ & Antennas that transmit an equal amount of energy in all directions in the horizontal plane are typically referred to as "omnidirectional antennas" or "non-directional antennas" in the context of their radiation pattern. In the horizontal plane, these antennas have a radiation pattern that is circular, meaning that they radiate power at a consistent level across 360 degrees. This characteristic makes them well-suited for applications where the direction of the receiving device may vary or is not fixed, such as mobile devices in wireless networks, FM broadcasting, and certain types of base stations. \
% \midrule \textbf{Ours} $\to$ & Antennas that transmit an equal amount of energy in the horizontal direction are called omnidirectional antennas. Here's why:\ &- Omnidirectional means radiating signal equally in all directions around a central axis. In this context, that central axis is typically vertical. So, they effectively broadcast horizontally in a circular pattern.\ &Let me contrast this with other antenna types:\ &- Directional antennas focus energy in a specific direction (like a spotlight), not horizontally equally.\ &- Sectorial antennas radiate strongly within a defined sector (slice) of a circle, not uniformly horizontal. \
% \midrule \textbf{Score} $\to$ & 1.9999856015 \
% \bottomrule
% \end{tabularx} }
% \end{figure}

% \begin{figure}[!t] 
%     % \caption{A case study comparing gpt-4 and gemma-2-it-9b-SimPO where the SimPO model gives a more structured output.}  \label{tab:qual}  
%     { \tt \footnotesize \begin{tabularx}{\linewidth}{r X} \toprule
%     \textbf{Input} $\to$ & Q: antennas that transmit an equal amount of energy in the horizontal direction are called  \\
%     \midrule \textbf{gpt4-turbo-1106-preview} $\to$ & Antennas that transmit an equal amount of energy in all directions in the horizontal plane are typically referred to as "omnidirectional antennas" or "non-directional antennas" in the context of their radiation pattern. In the horizontal plane, these antennas have a radiation pattern that is circular, meaning that they radiate power at a consistent level across 360 degrees. This characteristic makes them well-suited for applications where the direction of the receiving device may vary or is not fixed, such as mobile devices in wireless networks, FM broadcasting, and certain types of base stations. \\
%     \midrule \textbf{gemma-2-it-9b-SimPO} $\to$ & Antennas that transmit an equal amount of energy in the horizontal direction are called \textbf{omnidirectional antennas}. \\\\
%     & Here's why: \textbf{Omnidirectional} means radiating signal equally in all directions \textit{around} a central axis.  In this context, that central axis is typically vertical. So, they effectively broadcast horizontally in a circular pattern. \\\\
%     & Let me contrast this with other antenna types: \\
%     & - \textbf{Directional antennas} focus energy in a specific direction (like a spotlight), not horizontally equally.\\
%     & - \textbf{Sectorial antennas} radiate strongly within a defined sector (slice) of a circle, not uniformly horizontal. \\
%     \bottomrule 
% \end{tabularx} }  
% \end{figure}

\begin{figure}[!t] 

    { \tt \footnotesize \begin{tabularx}{\linewidth}{r X} \toprule
    & \textbf{Input} $\to$ \\
    & Q: Convert natural language into a list of turn-by-turn directions. Go west on I-10 until you hit the 101 then take it north. You will eventually see the Hollywood sign.  \\
    \midrule & \textbf{DPO} $\to$ \\
    & 1. Merge onto Interstate 10 westbound, heading straight if traveling northwise, maintaining awareness for fast lane position for an extended journey along I-10. \\
    & 2. Continue driving west on I-10 without deviation, adhering to traffic regulations and speed limits, focusing on maintaining smooth progress through urban areas and open countryside alike. \\
    & 3. Approximately 15 miles past downtown Los Angeles or after passing exit 9B for Hollywood Freeway (US-101 N), keep looking for signs indicating the US-101 North entrance ramp. This ramp typically lies between exits 8B (DTLA/MacArthur Park) and 9A (Silver Lake Ave). \\
    & 4. Signal appropriately when reaching the designated ramp merge area, ensuring safety first by checking mirrors, blind spots, and traffic conditions before entering US-101 Northbound. Blend seamlessly with traffic flowing onto the ramp. \\
    & 5. Once merged successfully onto US-101 North, continue driving. The freeway may wind through residential neighborhoods or offer scenic views, depending on your location within Los Angeles; remain alert for exit signs and changing road conditions. \\
    & 6. As you ascend the hills northward, keep an eye out for landmarks such as Griffith Observatory or the iconic Hollywood sign, which should eventually come into view high atop Mount Lee, signaling your approach to this famous Los Angeles landmark. Typically, this vista emerges around exit 24, Grantville Galleria, though visibility can be affected by fog or smog, so stay attentive even if you don't immediately see it. \\
    & 7. When you spot the Hollywood sign, use a safe pullover area or designated parking lot if available to stop and appreciate the view. If possible, confirm your location before ceasing travel to ensure you've reached your destination. Congratulations – you've followed the directions accurately, guiding yourself from I-10 to reaching the spectacular Hollywood sign via US-101 North. \\
    \midrule & \textbf{SimPO} $\to$  \\
    
    & 1. Get onto I-10 West  \\
    & 2. Travel on I-10 West until you reach Interstate 101 (Hollywood Freeway) \\
    & 3. Take Exit 7B towards Hollywood/Burbank \\
    & 4. Once on 101, travel north \\
    & 5. Continue on 101 North until you see the Hollywood sign. \\
    \bottomrule 
\end{tabularx} 
    \caption{A case study comparing \method with DPO under the Mistral-Instruct setting. \method generates more concise and clear instructions without unnecessary details compared to DPO.}  \label{tab:dpo_simpo_case_study}  }  
\end{figure}


==> Tables/final_models.tex <==
\begin{table}[t]
    \centering 
    
    \caption{The HuggingFace links of the final models trained with different preference optimization methods.}
    \begin{tabular}{ll}
        \toprule
    & Mistral Base 7B                                                \\ \midrule
    SFT   & \href{https://huggingface.co/princeton-nlp/alignment-handbook/zephyr-7b-sft-full}{alignment-handbook/zephyr-7b-sft-full}   \\
    DPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Base-SFT-DPO}{princeton-nlp/Mistral-7B-Base-SFT-DPO}    \\
    IPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Base-SFT-IPO}{princeton-nlp/Mistral-7B-Base-SFT-IPO}    \\
    KTO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Base-SFT-KTO}{princeton-nlp/Mistral-7B-Base-SFT-KTO}    \\
    ORPO  & \href{https://huggingface.co/princeton-nlp/kaist-ai/mistral-orpo-beta}{kaist-ai/mistral-orpo-beta}             \\
    R-DPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Base-SFT-RDPO}{princeton-nlp/Mistral-7B-Base-SFT-RDPO}  \\
    SimPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Base-SFT-SimPO}{princeton-nlp/Mistral-7B-Base-SFT-SimPO} \\ \midrule
          & Mistral Instruct 7B                                             \\ \midrule
    SFT   & \href{https://huggingface.co/princeton-nlp/mistralai/Mistral-7B-Instruct-v0.2}{mistralai/Mistral-7B-Instruct-v0.2}       \\
    DPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-DPO}{princeton-nlp/Mistral-7B-Instruct-DPO}  \\
    IPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-IPO}{princeton-nlp/Mistral-7B-Instruct-IPO}   \\
    KTO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-KTO}{princeton-nlp/Mistral-7B-Instruct-KTO}   \\
    ORPO  & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-ORPO}{princeton-nlp/Mistral-7B-Instruct-ORPO}  \\
    R-DPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-RDPO}{princeton-nlp/Mistral-7B-Instruct-RDPO}  \\
    SimPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Mistral-7B-Instruct-SimPO}{princeton-nlp/Mistral-7B-Instruct-SimPO} \\ \midrule
    & Llama3 Base 8B                                            \\ \midrule
    SFT   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT}{princeton-nlp/Llama-3-Base-8B-SFT}        \\
    DPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-DPO}{princeton-nlp/Llama-3-Base-8B-SFT-DPO}   \\
    IPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-IPO}{princeton-nlp/Llama-3-Base-8B-SFT-IPO}   \\
    KTO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-KTO}{princeton-nlp/Llama-3-Base-8B-SFT-KTO}   \\
    ORPO  & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-ORPO}{princeton-nlp/Llama-3-Base-8B-SFT-ORPO}  \\
    R-DPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-RDPO}{princeton-nlp/Llama-3-Base-8B-SFT-RDPO}   \\
    SimPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Base-8B-SFT-SimPO}{princeton-nlp/Llama-3-Base-8B-SFT-SimPO} \\ \midrule 
    & Llama3 Instruct 8B                                  \\ \midrule
    SFT   & \href{https://huggingface.co/princeton-nlp/meta-llama/Meta-Llama-3-8B-Instruct}{meta-llama/Meta-Llama-3-8B-Instruct}     \\
    DPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Instruct-8B-DPO}{princeton-nlp/Llama-3-Instruct-8B-DPO}   \\
    IPO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Instruct-8B-IPO}{princeton-nlp/Llama-3-Instruct-8B-IPO}   \\
    KTO   & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Instruct-8B-KTO}{princeton-nlp/Llama-3-Instruct-8B-KTO}    \\
    ORPO  & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Instruct-8B-ORPO}{princeton-nlp/Llama-3-Instruct-8B-ORPO}  \\
    R-DPO & \href{https://huggingface.co/princeton-nlp/princeton-nlp/Llama-3-Instruct-8B-RDPO}{princeton-nlp/Llama-3-Instruct-8B-RDPO}  \\
          \bottomrule
    \end{tabular}

    \end{table}
